A Closer Look at How Fine-tuning Changes BERT

Given the prevalence of pre-trained contextualized representations in today's NLP, there have been many efforts to understand what information they contain, and why they seem to be universally successful. The most common approach to use these representations involves fine-tuning them for an end task. Yet, how fine-tuning changes the underlying embedding space is less studied. In this work, we study the English BERT family and use two probing techniques to analyze how fine-tuning changes the space. We hypothesize that fine-tuning affects classification performance by increasing the distances between examples associated with different labels. We confirm this hypothesis with carefully designed experiments on five different NLP tasks. Via these experiments, we also discover an exception to the prevailing wisdom that "fine-tuning always improves performance". Finally, by comparing the representations before and after fine-tuning, we discover that fine-tuning does not introduce arbitrary changes to representations; instead, it adjusts the representations to downstream tasks while largely preserving the original spatial structure of the data points.

==> findings/original.tex <==
\subsection{Original Performances}\label{sec:original}

Before analyzing the fine-tuning process, let us first compare
the predictive performances for the original (\ie, before fine-tuning) representations
of different sizes. We find the best performance for
each original representation by training a two-layer neural
network as described in \Cref{sec:cls}. 

\paragraph{Larger representations help semantic tasks more.}
\Cref{tb:originals} summarizes the performance of the five
representations on the different tasks.  As expected,
the smaller representations
usually have lower performance than the larger ones,
indicating more parameters can encode more information.
Across the different capacities, we observe that the
improvements on semantic tasks (PS-role and PS-fxn) are
larger than the syntax tasks (POS-tagging and
Dependency). From \bertTiny to \bertBase, PS-fxn improves
$13.61\%$ ($74.14\%\to 87.75\%$) while POS-tagging only improves
$2.62\%$ ($90.76\%\to 93.39\%$).  
This large difference
suggests that semantic tasks are harder than syntactic
tasks. 
% \vs{Also the fact
% that for POS even a smaller representation gives high
% accuracy.}\yz{The best performance of PS-role is not
% \bertBase either.}
The former require representations 
with larger capacity.

% \vs{General comments:
% 1. There should be a space before an open parenthesis in all cases in the
% previous para. And also elsewhere.
% 2. Maybe it makes sense to order the rows as POS, DEP, PS-fxn and PS-role
% within each block in the table. This makes the task increasing in difficulty, so
% the numbers will all be decreasing withing each block.
% 3. What do we measure here? Is it accuracy or F score. Please check.
% }
% \yz{It is the accuracy}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\small
\begin{tabular}{@{}llrr@{}}
\toprule
Representation               & Task & Acc    & Std   \\ \midrule
\multirow{4}{*}{\bertTiny}   & POS  & 90.76 & 0.24 \\ 
                             & DEP  & 86.74 & 0.22 \\ 
                             & PS-fxn  & 74.14 & 1.42 \\
                             & PS-role   & 58.38 & 0.78 \\ \midrule
\multirow{4}{*}{\bertMini}   & POS  & 93.81 & 0.10 \\
                             & DEP  & 91.82 & 0.00 \\ 
                             & PS-fxn  & 82.45 & 1.07 \\
                             & PS-role   & 68.05 & 1.08 \\ \midrule
\multirow{4}{*}{\bertSmall}  & POS  & 94.26 & 0.13 \\
                             & DEP  & 92.93 & 0.14 \\ 
                             & PS-fxn  & 86.26 & 0.54 \\
                             & PS-role   & 74.22 & 1.03 \\ \midrule
\multirow{4}{*}{\bertMedium} & POS  & 94.40 & 0.08 \\
                             & DEP  & 92.54 & 0.14 \\ 
                             & PS-fxn  & 86.56 & 0.41 \\
                             & PS-role   & 76.28 & 1.00 \\ \midrule
\multirow{4}{*}{\bertBase}   & POS  & 93.39 & 0.31 \\
                             & DEP  & 89.39 & 0.08 \\ 
                             & PS-fxn  & 87.75 & 0.41 \\
                             & PS-role   & 74.49 & 0.84 \\ \bottomrule
\end{tabular}\caption{Performances of the five
    representations on different tasks before fine-tuning.
    These results come from the last layer of each
    representation model.}\label{tb:originals}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> overfitting.tex <==
\section{Overfitting}\label{sec:overfitting}
In this section, we will first briefly review the concept of
overfitting of a predictor. Then, we will introduce the
notion of representation learning overfitting, which is
distinugishable from the predictor overfitting.

\subsection{Predictor
Overfitting}\label{sec:predictor-overfitting}
A predictor overfits when it performs well on the training
set but generalizes badly. To put it formally, suppose
$e(D,\phi,f)$ is the empirical error of a learned predictor $f$
on the dataset $D$ using representation $\phi$, and
$\hat{e}(\mathbb{D},\phi,f)$ is the expected error of predictor
$f$ on exmples drawn from the distribution $\mathbb{D}$
using representation $\phi$. Here, $f$ could be a simple
one-layer neural network and $\phi$ could be \bertBase.
Then, the predictor $f$ overfits the training set
$D_{train}$ if
there is another predictor $f^{\prime}$ such that:
\begin{equation}
    \begin{aligned}
        &e(D_{train}, \phi, f) < e(D_{train},\phi,f^{\prime}) \\
        &\hat{e}(\mathbb{D},\phi, f) >
        \hat{e}(\mathbb{D},\phi, f^{\prime})
    \end{aligned}
\end{equation}

A predictor overfits because it memorizes the training set
and thus lose the generalization ability to unseen examples.
However, the predictor $f$ does not directly operates on the
examples, instead, it operates on the
representations $\phi$ of the examples. A predictor
memorizes the training set by memorizing its representation.
So, a more precise statement is \textit{$f$ overfits on the
representation $\phi$ of the dataset $D$.}

As pointed out by~\citet{zhou2021directprobe}, the
performance of a learning task is decided by two
sub-problems:
\begin{inparaenum}[(a)]
\item learning a representation and
\item learning a
predictor~\cite{DBLP:journals/pami/BengioCV13}.
\end{inparaenum}
Most of the previous work focus on
analyzing the preditor overfitting.\yz{need some citations
here} However, there is a missing part of the overfitting
analysis: the \textit{representation overfitting.} 

To illustrate the representation overfitting problem,
consider a simple feature vector whose first dimension is
the label index(starts from $1$) and the remaining
dimensions are the normal features designed for this task.
For unseen examples, the first dimension is always $0$.
When the predictor $f$ learns on this representation space,
it can easily achieve $100\%$ accuracy on the training set
because it can memorize the first dimension. However, this
predictor will perform poorly on unseen examples. This bad
performance can not be alleviated by adding a regularizer or
any other techniques because this is caused by the
representation overfitting not the predictor overfitting.

The representation overfitting problem was not prominent
because the representation space was usually
hand-crafted\yz{more citations}.
However, with the development of neural
networks~\cite{DBLP:conf/nips/YosinskiCBL14,
luong-etal-2015-effective}, pretrained
embeddings~\cite{DBLP:conf/nips/MikolovSCCD13,pennington-etal-2014-glove,devlin-etal-2019-bert} become the
standard practice. As a result, the problem of
representation overfitting becomes important.

\subsection{Representation Overfitting}

Given a learning task $(D,\phi,f)$, we seek to distinguish
the difference between:
\begin{inparaenum}[(a)]
\item the predictor $f$ overfits on the representation $\phi$ of the
    dataset $D$;
\item the representation $\phi$ overfits on the dataset $D$.
\end{inparaenum}
To fully isolate the performacne of $\phi$, a common
practice is to fix the $f$ by finding the best $f$ for
$\phi$. This paradigm is widely used for probing
representation
spaces~\cite{kim-etal-2019-probing,whitney2020evaluating,kim-etal-2019-probing}.

\paragraph{Empirical error of a representation}
Following the probing 
paradigm, we define the empirical error $e_R$ of a representation
$\phi$ on two datasets $D_0$ and $D_1$ as:

\begin{equation}
    e_{R}(D_0,D_1,\phi) = e(D_1, \phi, f^{*})
\end{equation}

$f^{*}$ is the best predictor can be learned from
$\phi(D_0)$:
\begin{equation}
    f^{*} =
    \min\limits_{f}\ell_T(D_0,\phi,f)\label{eq:best-func}
\end{equation}

where $\ell_T$ is a task-dependent loss function. In
practice, $D_0$ and $D_1$ could be the training set and test
set.

The empirical error of a representation $\phi$ is built on
two datasets because it needs a predictor to learn the
regularities expressed by the representation from one
dataset and test the learned regularities on another
dataset.

\paragraph{Training error of a representation} Suppose we
have a dataset $S$, which is used to train (pretrain or
fine-tuning) a representation:

\begin{equation}
    \phi_S^*=\min\limits_{\phi}\ell_P(S,\phi)\label{eq:pretrain}
\end{equation}

where $\ell_P$
is a pretraining loss function, \eg masked language
prediction.

Let $S_0,S_1\subset S, S_0\cap S_1=\emptyset$, then we
define the \textit{training error} of $\phi_S^{*}$ as the
empirical error $e_R(S_0,S_1,\phi_S^{*})$. Based on the
definitions, we know that $\phi_S^{*}$ is trained from both
$S_0$ and $S_1$ while the best predictor $f^{*}$ from
\Cref{eq:best-func} is only trained from $S_0$. As a result,
$S_1$ is only visible to the representation $\phi_S^{*}$.
Thus, $e_R(S_0,S_1,\phi_S^{*})$ can capture the training
performance of $\phi_S^{*}$ without being affected by the predictor
$f^{*}$ because $f^{*}$ never sees the $S_1$.

Be note, the $\ell_T$ in \Cref{eq:best-func} and $\ell_P$ in
\Cref{eq:pretrain} are not necessary to be the same, \eg
\bertBase is trained from masked language prediction but
being used for many different tasks.


\paragraph{Overfitting of a representation} Once we
estiblish the notion training error of a representation, we
can define the overfitting of a representation. Similar to
the predictor overfitting mentioned in
\Cref{sec:predictor-overfitting}, the
representation $\phi_S^{*}$ is overfitting if we can find
another representation $\phi^{\prime}$ such that:
\begin{equation}
    \begin{aligned}
        & e_R(S_0,S_1,\phi_S^{*}) < e_R(S_0,S_1,\phi^{\prime}) \\
        & \hat{e}_R(S_0,\mathbb{D}, \phi_S^{*}) >
        \hat{e}_R(S_0,\mathbb{D}, \phi^{\prime})
    \end{aligned}\label{eq:overfit-condition}
\end{equation}

where $\hat{e}_R(S_0,\mathbb{D},\phi)$ is the \textit{expected error}
of $\phi$, which is trained from $S_0$, on examples drawn
from distribution $\mathbb{D}$.


